Radial differential rotation leading to dipole collapse in pre-main-sequence stars

Despite progress in the observations of stellar magnetic fields, their physical mechanisms remain poorly understood. During the pre-main sequence (PMS) phase, the inner layers of stars contract and a radiative core gradually develops. In contrast, the convective envelope is gradually braked through magnetic interactions with the accretion disk and winds. With developing differential rotation inside the star, PMS phase is thus a critical period for magnetic properties of stars when strong initial dipoles can get perturbed, leading to the observed diversity in the magnetism on the main sequence (MS). In this work, we study the impact of differential rotation on such fields. We perform three-dimensional anelastic convective dynamo simulations of rotating spherical shells with an imposed differential rotation (shear) between the boundaries. Density, gravity profiles and convective zone thicknesses were set close to those predicted in PMS low-mass stars by one-dimensional stellar evolution code Cesam2k20. Our results show that radial differential rotation can induce dipole collapse leading to weaker, oscillatory magnetic fields. Differential rotation seems to perturb $\alpha^2$ dynamo mechanism, responsible for dipolar magnetic fields, by shearing poloidal field lines and by affecting turbulent magnetic transport processes. This collapse is moderated by the relative importance of shear compared to the vigor of convective motions, with exact stability criterion depending on the field strength and the size of the radiative core. Applying DNS-based stability criterion in PMS stellar evolution models, we qualitatively reproduce the trends observed in the magnetic topologies of low-mass stars when assuming an efficient internal angular momentum redistribution. This suggests that stellar magnetic properties are intimately related to the PMS angular momentum evolution.

==> 32_anna.tex <==
When the matter is distributed homogeneously in radius, $g\sim r$, convection is most vigorous near the outer shell, as shown by the distribution of $\Ross_{\rm conv}$ (Fig.~\ref{fig:cesam}b). This flow configuration corresponds to convective columns being the most pronounced at high radii, visible from the snapshots of equatorial cuts of radial velocity $u_r$ (Fig.~\ref{fig:cesam}d). This is different from the later stages of PMS stars which show more homogeneous distribution of $\Ross_{\rm conv}$, as well as the turbulent convective structures across the domain (Fig.~\ref{fig:cesam}c), for a fixed density contrast $N_\rho$. This is, however, valid only for convection with a gap $\xi=0.35$; for narrower gaps, convective columns become concentrated around the inner core (Fig.~\ref{fig:cesam}e) (see also \citet{Raynaud2014}). This variation in convection topology will affect the dynamo action known to be promoted by helicity. We observe that the distribution of helicity correlates with that of the convective Rossby number. 

\ludo{ The initial conditions correspond to dipolar dynamos already identified in \citet{GastineDW12}. Their parameter study has shown the effects of $Ra$, $N_\rho$ for two different aspect ratios on the stability of dipolar dynamos. Our parameter set is similar except that we consider higher values for $Pm$ in order to have stable dipolar dynamos with higher density contrast $N_\rho=2.5$ corresponding to realistic values for PMS stars. For the parameter regimes under consideration, dipolar dynamo solutions exist for the different gravity profiles in a certain window of $Ra$. Thie buoyant forcing must be sufficiently strong for dynamo action and sufficiently low to avoid dipole collapse induced by inertia. This window differs from one gravity profile to the other, but, the values normalized by the onset of convection $Ra_c$ are between $3$ and $10$ corresponding to turbulent flows with helical structures mainly located where gravity is maximum. It means that our parameter set and numerical setup enable us to consider different cases potnentially of interest for PMS stars.}

Extensive parameter studies show that differential rotation can give rise to different dynamical regimes in spherical Couette flows~\citep{wicht2014flow}. Here, we limit our attention to low values of the shear rates below the critical one for the shear instability and convection is the primary instability responsible for turbulent motions. We found that differential rotation affects convective columns insignificantly, slightly intensifying them at first and then suppressing at stronger rotations (see Fig.~\ref{fig:Roconv_varom}).

==> intro.tex <==
Pre-main-sequence (PMS) stars form as a result of the gravitational collapse of molecular clouds. This process involves three stages (a) fully embedded phase - class 0, (b) class I, (c) class II and (d) \lm{weak} T Tauri stars, where the star is entirely separated from the disc (class III). Spectropolarimetric observations (Nicholson 2021, Alecian ?) of pre-main-sequence low-mass stars indicate that younger stars are more likely to possess large-scale dipolar magnetic fields than older ones \lm{[[it seems that we find the opposite with cesam models...]]}. These results suggest that stellar dynamo, generation of magnetic fields by developing convective motions \lm{[in rotation?]}, can be affected by the changing conditions on the stellar surface during stellar formation. Indeed, regions of increased temperature (accretion shocks) are thought to develop at the surface of the protostar, with two scenarios proposed: equatorial accretion when magnetic field is weak or non-existent, and pole-ward accretion when the mass flux of accreted particles is directed along the field lines of a strong, dipolar magnetic field \anna{[cite]}. The gravitational pull of the disc could also potentially influence dynamo action through radially asymmetric gravity profile \anna{[cite].}

However, perhaps the main impact on the magnetic topology could result from the core contraction and increase of the differential rotation in the core. Consider that angular momentum is distributed more or less equally through transport by convection and that there is no net angular momentum transport. When the core begins to collapse, this should result in speed-up of the inner parts of the star and of the developing radiative core, when the outer part is still rotationally locked to the disk. \anna{This phenomenon is well captured in stellar evolution models, where differential rotation in the core can increase up to XX times from the start of the model, typically at T Tauri phase, to the arrival of the star to the main sequence [cite].}  On the other hand, dynamo theory and numerical simulations show that differential rotation results in decreasing the relative dipole strength (dipolarity parameter) and drives magnetic cycles through so-called oscillatory dynamos~\citep{parker1955hydromagnetic,yoshimura1975solar,schrinner2012dipole}.

\ludo{
One of the most striking features of PMS stars is their diverse rotation rates.
Observations of young clusters (ages of a few Myr up to $\sim$20-30 Myr) show a broad spread in rotation periods, ranging from very slow rotators (tens of days) to very fast ones (a few tenths of a day). This spread reflects both initial conditions and the interplay of processes that act to spin-up or spin-down during the PMS phase \citep{scholz2007rotation}. Magnetism plays a central role in regulating rotation in PMS stars, but, magnetic effects depend on field strength and magnetic topologies. Young PMS stars, particularly T-Tauri stars, can possess strong magnetic fields (kilogauss scale) which can interact with their circumstellar disks. This star-disk coupling can act as a brake (``disk locking'') that removes angular momentum from the star, slowing its rotation despite contraction \citep{bouvier2014angular}.

Theoretical models must account for several competing processes: contraction, disk locking/star-disk interaction, magnetized stellar winds, and internal angular momentum transport \citep{galli2015angular}. This redistribution of angular momentum induces large-scale differential rotation known to play a crucial role through the $\Omega$-effect in generating magnetic fields \citep{Moffatt78}. But, it can also perturb the pattern of convective cells present in a huge part of their interior.

Observational constraints are improving thanks to rotation periods from spot modulation, vsini surveys, Zeeman‑Doppler imaging to reconstruct large‑scale magnetic topologies, and measurements of X-ray or H$\alpha$ activity as proxies of magnetic fields \citep{donati2007magnetospheric,gregory2012magnetic}. PMS stars are shaped by the interplay between contraction (forcing spin-up), and magnetic effects (disk locking, wind braking) that act to slow or regulate rotation. Understanding these processes is crucial because the PMS sets the initial conditions (rotation, magnetism, core/envelope structure) for main-sequence evolution, which in turn affects magnetic activity lifetimes, spin-down behaviour, and even planet formation.

PMS stars are very rich systems from a physical point of view in which a diversity of physical processes operate on different timescales. Taking into account all of them is not a possible task for actual 3D simulations. Instead, we focus on the stability of dipolar dynamos driven by convection in a thick rotating spherical enveloppe influenced by large-scale differential rotation as it is expected for convective zones of PMS stars located between a contracting core and a stellar surface braked by the star-disk interaction. This work aims to explore in detail the combined effects of rotation and magnetism during the PMS phase, focusing on  how magnetic field strength and topology change as the internal structure transitions and  ultimately set the “initial rotational distribution” entering the main sequence.
}

In this work, we elucidate how differential rotation affects magnetic field generation in convective zones of the pre-main-sequence stars, and establish a criterion for collapse of large-scale dipole field for stellar evolution code \cesamxx \citep[Manchon et al., subm.]{Morel1997,Morel2008,Marques2013}. In section 2, we discuss the numerical setup, governing and diagnostic parameters of the magnetohydrodynamic dynamo model. In section 3, we discuss magnetic field evolution and mechanisms of the dipole collapse in the presence of differential rotation.  In section 4, we propose a local and global criteria for the dipole stability based on the radial component of the differential rotation in the stars. In section 5, we analyse \lm{the predictions of} this criterion on grids of 1D stellar models from \cesamxx code, and derive resulting implications for stellar magnetic topologies.
